Extracted BERT Model Leaks More Information than You Think!

The collection and availability of big data, combined with advances in pre-trained models (e.g. BERT), have revolutionized the predictive performance of natural language processing tasks. This allows corporations to provide machine learning as a service (MLaaS) by encapsulating fine-tuned BERT-based models as APIs. Due to significant commercial interest, there has been a surge of attempts to steal re mote services via model extraction. Although previous works have made progress in defending against model extraction attacks, there has been little discussion on their performance in preventing privacy leakage. This work bridges this gap by launching an attribute inference attack against the extracted BERT model. Our extensive experiments reveal that model extraction can cause severe privacy leakage even when victim models are facilitated with advanced defensive strategies.

==> tab-aia.tex <==
\begin{table}
\scalebox{0.85}{
% \small
% \begin{center}
% \begin{wraptable}[]
     \centering
    \begin{tabular}{cccc}
         \hline
       & AG news & Blog & TP-US\\
         \toprule
Majority class & 49.94 & 49.57 & 38.15 \\
\midrule
BERT (w/o fine-tuning)&  69.39 &  44.03 & 49.38\\
\midrule
$\mathcal{T}_A=\mathcal{T}_V$ ($D_V$) &   22.74  &  36.37&  36.76\\
\midrule
$\mathcal{T}_A = \mathcal{T}_V$ ($D_A$)\\

1x  &   21.01  & 35.98 &  37.34\\
\midrule
$\mathcal{T}_A \neq \mathcal{T}_V$ (reviews)\\
       1x  &   17.93 &  34.34  & \textbf{35.97} \\
        5x &  18.31 &  34.45&  36.82 \\
\midrule
$\mathcal{T}_A \neq \mathcal{T}_V$ (news)\\
        1x  &    \textbf{15.76} & \textbf{33.88}	& 36.92 \\
        5x  &   17.91	&  35.39	&37.68 \\
% \midrule
% $D_A \rightarrow D_V$ &   18.61 &   34.78  &37.70 \\
\bottomrule
    \end{tabular}}
    \vspace{3pt}
    \caption{%Privacy protection of attribute inference %(privacy) 
    AIA attack success over different datasets. The extracted model is trained on the queries from different distributions, and the attribute inference model is trained on the public data $D_A$ (\cf Algorithm~\ref{Algorithm:aia}). Note higher value means better empirical privacy.%, \ie lower attack success. %(2nd half: $D_A$ reserved for the training of AIA attack model.% to mount AIA).
    }
    % \vspace{-20pt}
    \label{tab:aia}
\end{table}
%\vspace{-5mm}
% \end{wraptable}

==> tab-att_acc.tex <==
\begin{table}[t]
\scalebox{0.535}{
    \centering
    \begin{tabular}{cccccc}
    \hline
     \multicolumn{6}{c}{\resource{ag} news}\\
     \hline
        	& {\makecell{entity 0 \\(std=310.0)}}	& {\makecell{entity 1 \\(std=1568.5)}}	&{\makecell{entity 2 \\(std=2095.5)}}	& {\makecell{entity 3 \\(std=2640.5)}}	& {\makecell{entity 4 \\(std=2615.5)}}\\
        	\hline
$\mathcal{T}_A=\mathcal{T}_V$	& 15.61 &    15.10	&  7.71	&   6.95	& 5.49 \\
\makecell{$\mathcal{T}_A \neq \mathcal{T}_V$ \\(news)} 
& 14.79	& 12.38	& 3.84	& 5.33	&2.02\\ \hline
% \multicolumn{5}{c}{} \\
% \hline
& \multicolumn{2}{c|}{\resource{tp-us}} & \multicolumn{2}{c}{Blog} \\
\hline
	& {\makecell{gender \\(std=1512.0)}}	&\multicolumn{1}{c|}{{\makecell{age \\(std=1440.0)}}} %&		
	&{\makecell{age \\(std=28.0)}}	&{\makecell{gender \\(std=6.0)}} \\
$\mathcal{T}_A=\mathcal{T}_V$	& 36.40& \multicolumn{1}{c|}{37.12}	& %$\mathcal{T}_A=\mathcal{T}_V$	& 
32.18	& 39.02\\
\makecell{$\mathcal{T}_A \neq \mathcal{T}_V$ \\(reviews)}&	36.44	&\multicolumn{1}{c|}{37.40}	& %$\mathcal{T}_A \neq \mathcal{T}_V$ \\(reviews) &
31.20	&38.01\\
\hline
    \end{tabular}}
    \vspace{3pt}
    \caption{%The accuracy of the individual attributes of the attackers on extracted models 
    AIA performance on attributes of different datasets. All experiments are based on 1x queries. std is the standard deviation of attribute distribution.}
    \label{tab:att_acc}
\end{table}

==> tab-att_acc_ijcai.tex <==
\begin{table}[t]
\scalebox{0.67}{
    \centering
    \begin{tabular}{cccccc}
    \hline
     \multicolumn{6}{c}{\resource{ag} news}\\
     \hline
        	& {\makecell{entity 0 \\(std=310.0)}}	& {\makecell{entity 1 \\(std=1568.5)}}	&{\makecell{entity 2 \\(std=2095.5)}}	& {\makecell{entity 3 \\(std=2640.5)}}	& {\makecell{entity 4 \\(std=2615.5)}}\\
        	\hline
$\mathcal{T}_A=\mathcal{T}_V$	& 15.61 &    15.10	&  7.71	&   6.95	& 5.49 \\
\makecell{$\mathcal{T}_A \neq \mathcal{T}_V$ \\(news)} 
& 14.79	& 12.38	& 3.84	& 5.33	&2.02\\ \hline
% \multicolumn{5}{c}{} \\
% \hline
& \multicolumn{2}{c|}{\resource{tp-us}} & \multicolumn{2}{c}{Blog} \\
\hline
	& {\makecell{gender \\(std=1512.0)}}	&\multicolumn{1}{c|}{{\makecell{age \\(std=1440.0)}}} %&		
	&{\makecell{age \\(std=28.0)}}	&{\makecell{gender \\(std=6.0)}} \\
$\mathcal{T}_A=\mathcal{T}_V$	& 36.40& \multicolumn{1}{c|}{37.12}	& %$\mathcal{T}_A=\mathcal{T}_V$	& 
32.18	& 39.02\\
\makecell{$\mathcal{T}_A \neq \mathcal{T}_V$ \\(reviews)}&	36.44	&\multicolumn{1}{c|}{37.40}	& %$\mathcal{T}_A \neq \mathcal{T}_V$ \\(reviews) &
31.20	&38.01\\
\hline
    \end{tabular}}
    %\vspace{-3pt}
    \caption{%The accuracy of the individual attributes of the attackers on extracted models 
    AIA performance on attributes of different datasets. All experiments are based on 1x queries. std is the standard deviation of attribute distribution.}
    \label{tab:att_acc}
%\vspace{-5pt}
\end{table}

==> tab-data.tex <==
\begin{table}[!htp]
\scalebox{0.7}{
    \centering
% \resizebox{\columnwidth}{!}{
    \begin{tabular}{llllll}
    \hline
Dataset & Private Variable & \#Train & \#Dev& \#Test & Category  \\
    \toprule
%      en-de &4.2M & 3000 & 3003\\
\resource{tp-us} & age, gender & 22,142  & 2,767 & 2,767 & SA \\
\resource{ag} & entity & 11,657 & 1,457 &1,457  & TC\\
\resource{ag} full & - & 112k & 1,457 & 1,457 & TC\\
Blog & age, gender & 7,098 &887 &887 & TC\\
Yelp & - & 520k & 40,000 & 1,000 & SA \\
      
     \bottomrule
 \end{tabular}}
%  }
    % \vspace{3pt}
    \caption{Summary of NLP datasets. SA: sentiment analysis; TC: topic classification.}
    \label{tab:data}
\end{table}

==> tab-data_ijcai.tex <==
\begin{table}[!htp]
 \centering
 \scalebox{0.87}{
% \resizebox{\columnwidth}{!}{
    \begin{tabular}{llllll}
    \hline
Dataset & Private Variable & \#Train & \#Dev& \#Test & Category  \\
    \toprule
%      en-de &4.2M & 3000 & 3003\\
\resource{tp-us} & age, gender & 22,142  & 2,767 & 2,767 & SA \\
\resource{ag} & entity & 11,657 & 1,457 &1,457  & TC\\
\resource{ag} full & - & 112k & 1,457 & 1,457 & TC\\
Blog & age, gender & 7,098 &887 &887 & TC\\
% Yelp & - & 520k & 40,000 & 1,000 & SA \\
      
     \bottomrule
 \end{tabular}
  }
    % \vspace{3pt}
    \caption{Summary of NLP datasets. SA: sentiment analysis; TC: topic classification.}
    \label{tab:data}
\end{table}

==> tab-mea_full.tex <==
\begin{table}[t]
\scalebox{0.75}{
    \centering
    \begin{tabular}{c|ccccc}
    \hline
       & AG news & {\makecell{AG news \\(full)}} & Blog & TP-US & Yelp\\
         \hline
     Victim model & 79.99 & 94.47 & 97.07 &  85.53 & 95.57\\
         \hline\hline
  \makecell{$\mathcal{T}_A=\mathcal{T}_V $\\($D_V$)} &  \textbf{80.83} & \textbf{94.54}  & \textbf{96.77} &  86.48 & \textbf{95.72} \\
        \makecell{$\mathcal{T}_A=\mathcal{T}_V$ \\($D_A$)} &  80.10 & 94.38 & 95.64 & \textbf{86.53} & 95.61\\
        \hline\hline
    \makecell{$\mathcal{T}_A \neq \mathcal{T}_V$ \\(reviews)}\\
         \hline
         0.1x & 50.90 & 86.57 &  36.83& 79.95  & 92.39 \\
        0.5x & 68.13 & 87.31 &84.59  & 84.21  & 93.25\\
       1x  &  69.94 & 88.63 & 88.16 &  85.15 & 94.06 \\
        5x &  75.29& 91.27 & 92.75 &  85.82 & 94.95 \\
        \hline\hline
         \makecell{$\mathcal{T}_A \neq \mathcal{T}_V$ \\(news)}\\
         \hline
          0.1x & 61.70 & 89.13 &18.04  & 79.20  & 88.24\\
        0.5x & 70.56 & 89.84 & 32.92 & 84.18  & 89.76\\
        1x  &  71.95  & 90.47 & 83.13	&  84.15	& 91.06 \\
        5x  &   75.82 	&92.26 & 87.64	& 85.46	& 93.13 \\
        \hline
    \end{tabular}}
    \vspace{3pt}
    \caption{Accuracy of victim models and extracted models %among different datasets in terms of 
    across different domains and query sizes. %Note the high accuracies for some tasks even at low query budgets, and diminishing accuracy gains at higher budgets.
    }
    \label{tab:mea_full}
\end{table}

==> tab-mea_full_ijcai.tex <==
\begin{table}[t]
\scalebox{0.8}{
    \centering
    \begin{tabular}{c|ccccc}
    \hline
       & AG news & {\makecell{AG news \\(full)}} & Blog & TP-US & Yelp\\
         \hline
     Victim model & 79.99 & 94.47 & 97.07 &  85.53 & 95.57\\
         \hline\hline
%   \makecell{$\mathcal{T}_A=\mathcal{T}_V $\\($D_V$)} &  \textbf{80.83} & \textbf{94.54}  & \textbf{96.77} &  86.48 & \textbf{95.72} \\
        \makecell{$\mathcal{T}_A=\mathcal{T}_V$ ($D_{Q}$)} &  \textbf{80.10} & \textbf{94.38} & \textbf{95.64} & \textbf{86.53} & \textbf{95.61}\\
        \hline\hline
    \makecell{$\mathcal{T}_A \neq \mathcal{T}_V$ (reviews)}\\
         \hline
         0.1x & 50.90 & 86.57 &  36.83& 79.95  & 92.39 \\
        0.5x & 68.13 & 87.31 &84.59  & 84.21  & 93.25\\
       1x  &  69.94 & 88.63 & 88.16 &  85.15 & 94.06 \\
        5x &  75.29& 91.27 & 92.75 &  85.82 & 94.95 \\
        \hline\hline
         \makecell{$\mathcal{T}_A \neq \mathcal{T}_V$ (news)}\\
         \hline
          0.1x & 61.70 & 89.13 &18.04  & 79.20  & 88.24\\
        0.5x & 70.56 & 89.84 & 32.92 & 84.18  & 89.76\\
        1x  &  71.95  & 90.47 & 83.13	&  84.15	& 91.06 \\
        5x  &   75.82 	&92.26 & 87.64	& 85.46	& 93.13 \\
        \hline
    \end{tabular}}
    %\vspace{3pt}
    \caption{Accuracy of victim models and extracted models %among different datasets in terms of 
    across different domains and query sizes. %Note the high accuracies for some tasks even at low query budgets, and diminishing accuracy gains at higher budgets.
    }
    \label{tab:mea_full}
    \vspace{-5pt}
\end{table}

==> tab-overlap_emnlp.tex <==
\begin{table}[t]
\scalebox{0.65}{
    \centering
    \begin{tabular}{lcc|cc|cc}
    \hline
Query   &   \multicolumn{2}{c}{AG news (full)} & \multicolumn{2}{c}{Blog} & \multicolumn{2}{c}{TP-US} %& \multicolumn{2}{c}{Yelp}
\\
         \toprule
         
    &     uni-gram & 5-gram &uni-gram & 5-gram & uni-gram & 5-gram %&uni-gram & 5-gram 
    \\
           \midrule
reviews   & 68.22\% &0.53\% & 47.21\% & 0.73\% & 60.86\% & 2.57\%\ %& 52.68\% & 2.64\% 
\\
       
news  & 72.13\% & 1.24\% & 44.76\% & 0.06\% & 51.28\% & 0.12\% %& 38.69\% & 0.19\% 
\\
    \hline
    \end{tabular}}
    %\vspace{-3pt}
    \caption{Percentage of uni-gram and 5-gram recall-based overlap between different queries and test sets. Since AG news is derived from AG news (full) and they show a similar distribution, we omit it.%Note the high accuracies for some tasks even at low query budgets, and diminishing accuracy gains at higher budgets.
    }
    %\vspace{-5mm}
    \label{tab:overlap}
    %\vspace{-10pt}
\end{table}

==> tab-overlap_ijcai.tex <==
\begin{table}[t]
\scalebox{0.75}{
    \centering
    \begin{tabular}{lcc|cc|cc}
    \hline
Query   &   \multicolumn{2}{c}{AG news (full)} & \multicolumn{2}{c}{Blog} & \multicolumn{2}{c}{TP-US} %& \multicolumn{2}{c}{Yelp}
\\
         \toprule
         
    &     uni-gram & 5-gram &uni-gram & 5-gram & uni-gram & 5-gram %&uni-gram & 5-gram 
    \\
           \midrule
reviews   & 68.22\% &0.53\% & 47.21\% & 0.73\% & 60.86\% & 2.57\%\ %& 52.68\% & 2.64\% 
\\
       
news  & 72.13\% & 1.24\% & 44.76\% & 0.06\% & 51.28\% & 0.12\% %& 38.69\% & 0.19\% 
\\
    \hline
    \end{tabular}}
    %\vspace{-3pt}
    \caption{Percentage of uni-gram and 5-gram recall-based overlap between different queries and test sets. Since AG news is derived from AG news (full) and they show a similar distribution, we omit it.%Note the high accuracies for some tasks even at low query budgets, and diminishing accuracy gains at higher budgets.
    }
    %\vspace{-5mm}
    \label{tab:overlap}
    %\vspace{-10pt}
\end{table}
